Wasserstein Barycenter-based Model Fusion and Linear Mode Connectivity of Neural Networks

Based on the concepts of Wasserstein barycenter (WB) and Gromov-Wasserstein barycenter (GWB), we propose a unified mathematical framework for neural network (NN) model fusion and utilize it to reveal new insights about the linear mode connectivity of SGD solutions. In our framework, the fusion occurs in a layer-wise manner and builds on an interpretation of a node in a network as a function of the layer preceding it. The versatility of our mathematical framework allows us to talk about model fusion and linear mode connectivity for a broad class of NNs, including fully connected NN, CNN, ResNet, RNN, and LSTM, in each case exploiting the specific structure of the network architecture. We present extensive numerical experiments to: 1) illustrate the strengths of our approach in relation to other model fusion methodologies and 2) from a certain perspective, provide new empirical evidence for recent conjectures which say that two local minima found by gradient-based methods end up lying on the same basin of the loss landscape after a proper permutation of weights is applied to one of the models.

==> Wasserstein Barycenter-based Model Fusion and Linear Mode Connectivity of Neural Networks/experiments.tex <==
\section{Experiments}\label{section: experiment}

{\textbf{Overview:}
We present an empirical study of our proposed WB and GWB based fusion algorithms to assess its performance in comparison to other state of the art fusion methodologies and reveal new insights about the loss landscapes for different types of network architectures and datasets. We first consider the fusion of models trained on heterogeneous data distributions.
% and show that for certain combinations our fused model outperforms the base models. 
Next we present results for WB fusion of FC NNs and deep CNNs, and draw connections between workings of WB fusion and LMC of SGD solutions. 
Finally, we consider GWB fusion and present results on RNNs, LSTMs and extend the conjecture made in \cite{entezari2021role} for recurrent NNs.}

%We first present the results of model fusion for different network architectures and datasets under both WB and GWB based fusion frameworks. In particular, for WB based method, we show the results on fully connected NNs and deep convolutional models like VGG11 and $\resnet$. And for GWB based method, we present the results on RNNs and LSTMs (other relevant experiments like single shot model distillation and knowledge transfer based on our fusion method can be found in the Supplement). Secondly, we visualize the fusion results of both two frameworks on two-dimensional subspace of the loss surface of NNs. By the visualizations, we explain the mechanisms behind of fusion algorithms and make connections to the conjecture in \cite{entezari2021role}.}

{\textbf{Baselines:} 
For baselines, we consider vanilla averaging and the state-of-the-art fusion methodologies like OT fusion \cite{singh2019model} and FedMA \cite{wang2020federated}. For a fair comparison under the experimental settings of one-shot fusion we consider FedMA without the model retraining step and restrict its global model to not outgrow the base models. We refer to this as ``one-shot FedMA''. For RNNs and LSTMs, our baselines additionally include slightly modified versions of WB based fusion and OT fusion where we ignore the hidden-to-hidden connections. Other methods which require extensive training are not applicable in one-shot model aggregation settings. }
% {\red We also leave the potential applications of our fusion method in federated learning settings \cite{mcmahan2017communication} for future work.
% }}

\textbf{Base models \& General-setup:} For our experiments on FC NNs, we use $\mlp$ introduced in \cite{singh2019model}, which consists of 3 hidden layers of sizes $\{400, 200, 100\}$. Additionally, we introduce $\mlpl$ and $\mlps$ with hidden layers of size $\{800, 400, 200\}$ and $\{200, 100, 50\}$ respectively.
For deep CNNs, we use VGG11 \cite{simonyan2014very} and $\resnet$ \cite{he2016deep}. For recurrent NNs, we work with RNNs and LSTMs with one hidden layer of size $256$ and $4 \times 256$ respectively.
Hyperparameters are chosen using a validation set and final results are reported on a held out test set. More training details are provided in the Appendix. 
% {\red For all loss landscape visualizations we fuse two base models and initialize the target model using the first base model.}

{\textbf{Visualization methodology:} 
We visualize the result of fusing two pre-trained models on a two-dimensional subspace of NNs' loss landscape by using the method proposed in \cite{garipov2018loss}.
In particular, each plane is formed by all affine combinations of three weight vectors corresponding to the parameters of base model 1, base model 2 and permuted model 2 (i.e. base model 2 \textit{after} multiplying its weights by the coupling obtained by our fusion algorithm) respectively.
}

%{\red \textbf{General setup:} Hyperparameters are chosen as the best performing ones on the validation set while the final results are reported on a held out test set. More details on model training and hyperparameters used is provided in the Supplement. For the visualizations, we always consider fusing two based models, and the target model is initialized using one of the base models.}


% \subsection{Experiments on WB based fusion}\label{sec: experiments on WB based fusion}

%{\red
%In this section, we first demonstrate the use of WB-based framework
%for fusing fully connected NNs. In particular, for base models, we follow \cite{singh2019model} and train $\mlp$, which consists of $3$ hidden layers of sizes $400$, $200$ and $100$, on MNIST dataset. We consider fusion of $2$ independent trained models (see fusion of multiple model counts in the Supplement). The target model is set to be either have the same architecture as base models ($\mlp$) or be two times larger than base models (denoted as $\mlpl$, which consists of $3$ hidden layers of sizes $800$, $400$ and $200$). The second scenario can arise in the federated learning due to the limitation of memory and computational resources on edge devices. When fusing models into same architecture, we consider initialize the target model either using one of the base models or just randomly. When fusing models into larger architecture, the target model is initialized by random. Secondly, we apply our framework to fuse commonly used deep CNNs like VGG11 and $\resnet$, 
%trained till convergence on standard image classification dataset CIFAR10 \cite{krizhevsky2009learning}. Our framework easily incorporates the kernels in convolutional filters and skip connections in ResNet models (see the details in the Supplement). Here, we again consider the fusion of $2$ model counts, and the target model is initialized using one of the base models.}

% {\red \subsection{Aggregating models trained on heterogeneous data distributions}}
\subsection{WB fusion under heterogeneous data distributions}\label{sec: WB hetero}
\textbf{Setup:}  
We first apply WB fusion in aggregating models trained on heterogeneous data distributions which is a setting often found in federated learning where the clients have local data generated from different distributions and privacy concerns prevent data sharing among them. Here we follow the setup described in \cite{singh2019model}. To simulate heterogeneous data-split on MNIST digit classification one of the models (named A) is trained with a special skill to recognize one of the digits (eg. digit 4) that is not known to the other model, named B. Model B is trained on $90\%$ of the training data for remaining digits while model A uses the other $10\%$ data. Under this data split, we consider two settings. For the first setting, the base models are fused into a target model of the same architecture ($\mlp$). For the second setting, we consider the fusion of two small base models ($\mlps$) into a large target model ($\mlp$). This simulates the setting where clients in federated learning are constrained by memory resources to train smaller models. 
{In both cases we use model fusion to aggregate knowledge learned from the base models into a single model, a more memory-efficient strategy than its ensemble-based counterparts}. 
%When the target model is of the same architecture as the base model we randomly choose one of the base models to initialize {\red the weights of} the target model before starting the fusion. However when the target model has a different architecture the base model cannot be directly used and hence we propose an additional initialization step. In this additional step, we run one-shot model fusion on a single base model and a randomly initialized target model. The resulting target model is used as initialization for the subsequent fusion algorithm. We refer to this as distillation initialization. 
% {\red For fair comparison, we also apply the distillation initialization on OT fusion, which is not mentioned in \cite{singh2019model}. If we random initialize the target model for OT fusion (the way from the original paper), the test accuracy of the fused model obtained by OT fusion will be bad.}

\textbf{Quantitative results:} Figure \ref{fig: heterogeneous data distribution} shows the results of single shot fusion when different proportions of the base models are considered. We find that (a) WB fusion consistently outperforms the baselines,
%the fused models obtained from our WB algorithm consistently outperforms the baselines, 
(b) for certain combinations WB produces fused models with accuracy even better than the base model and demonstrates successful one shot knowledge aggregation. Note that for each proportion of model aggregation (x-axis),  the results are reported over multiple runs where one of the base models is randomly chosen to initialize the target model in the fusion algorithm.
% This is slightly different from \cite{singh2019model} where the target model is always initialized using model A and accounts for the differences when comparing against the plots in \cite{singh2019model}. 
We find that WB fusion is more stable against initialization as indicated by the lower variance in Figure \ref{fig: heterogeneous data distribution}. For fusion into different architectures vanilla averaging is not applicable, and we do not include ``one-shot FedMA'' for comparison here since it is not clear how to assign different proportions to base models in FedMA, or to specify a target architecture different from the base models.

\begin{figure}[!htb]
    \centering
    \begin{subfigure}{.4\textwidth}%
    \includegraphics[width=1.0\linewidth]{pics/Heterogeneous_Fusion_MNIST.png}
    \end{subfigure}%
    \begin{subfigure}{.4\textwidth}
    \includegraphics[width=1.0\linewidth]{pics/Heterogeneous_Fusion_MNIST_diff_arch.png}
    \end{subfigure}
\caption{\textbf{Left / Right:} Test accuracy \% for fused models when base models are trained on heterogeneous data distributions and combined with various proportions into a target model of \textbf{same / different} architecture. Some models obtained by WB fusion outperform even the base models.}
\label{fig: heterogeneous data distribution}
\end{figure}


\subsection{WB fusion under homogeneous data distributions and connections to LMC}\label{sec: WB homo}



{\textbf{Setup:} 
In this section we perform WB fusion for various models and architectures, and provide loss landscape visualizations which reveal workings of the fusion algorithm and shed light on linear model connectivity (LMC) of SGD solutions after applying appropriate permutations. We first consider fusion of FC NNs on the MNIST dataset \cite{deng2012mnist} and train $\mlp$ following \cite{singh2019model}. For this we consider two different settings. In the first setting, the target model has the same architecture as the base models. For the second one, we fuse the base models into a larger model $\mlpl$. As noted before, the latter scenario is relevant for federated learning, given the limitations of memory and computational resources on edge devices. Next, we consider fusion of deep CNNs like VGG11, $\resnet$ trained on CIFAR10 dataset \cite{krizhevsky2009learning}. For all these cases, we fuse 2 trained models initialized differently. For the skip-connection and fusion into different architectures, FedMA is not directly applicable and hence not considered for comparisons.}


{\textbf{Quantitative results:} Table \ref{table: WB fusion comparison} contains the results of fusion for FC NNs and deep CNNs. We find that (a) WB fusion produces models at par or outperforms other fusion methods for all considered model types and datasets, (b) for fusion into different architectures and ResNets, we find that WB fusion is more effective and robust.}
% {\red We attribute these to the fact that, in comparison to OT fusion, our algorithm iterates until convergence (see more details in the Appendix). }}
%{\red contains the results of single shot model fusion for fully connected NNs and deep CNNs. 
%(a) We find that WB fusion outperforms 
%other fusion types irrespective of model types and datasets. (b) When considering the hard settings like fusing into different architectures or the base models being deep neural networks, the WB fusion is more robust to the initialization of target model. This is because, compared to OT fusion, our fusion algorithm iterates until convergence, which eliminates the randomness from the initialization.}

\begin{table}[!htb]
	\caption{Performance comparison (Test accuracy $\pm$ standard deviation \%) of different fusion algorithms under various network architectures and datasets. ``BASE'' means initializing target model with one of the base models. For each case, the target model obtained by WB fusion gets the highest test accuracy and smallest standard deviation.}
	\label{table: WB fusion comparison}
	\centering
	\renewcommand\arraystretch{1.5}
	\resizebox{0.7\textwidth}{!}{
		\begin{sc}
			\begin{tabular}{@{}cccccc@{}}
				%\toprule
				& \multicolumn{2}{c}{MNIST} & \phantom{ab}& \multicolumn{2}{c}{CIFAR10}  \\ 
				\cmidrule{2-3} \cmidrule{5-6} 
				&  $\mlp$/base & $\mlpl$ & & VGG11/base & $\resnet$/base  \\ 
				\midrule
				Base Model Avg & $98.31 \pm 0.02$ & - & & $90.14 \pm 0.19$ & $91.56 \pm 0.34$ \\
				\midrule[0.05pt]
				Vanilla Avg & $86.50 \pm 4.60$ & - & & $30.82 \pm 4.49$ & $20.56 \pm 3.90$ \\
				One-shot FedMA & $97.89 \pm 0.10$ & - & & $\bm{85.42 \pm 1.01}$ & - \\
				OT & $97.84 \pm 0.12$ &  $91.53 \pm 2.64$& & $85.39 \pm 0.93$ & $71.37 \pm 6.53$ \\
				WB & $97.92 \pm 0.12$&  $\bm{94.93 \pm 1.18}$ & & $85.39 \pm 0.93$ &  $\bm{73.75 \pm 4.39}$ \\
				\bottomrule
			\end{tabular}
		\end{sc}
	}
\end{table}

\textbf{Visualizations:} 
Figure \ref{fig: visualization of FCNN training on MNIST and illustration of FCNN} (left) contains the visualization of fusing two $\mlp$ trained on MNIST dataset under WB framework and Figure \ref{fig: visualization of fusion results for different types of models and datasets} (left) contains the fusion result of WB fusion of two VGG11 models trained on CIFAR10. We find that (a) the couplings obtained in WB fusion (refer to equation \ref{eq: problem after plugging in cost function d_W}) between the layers of target model and base models are sparse, i.e. they are almost permutations; (b) the basins of the permuted model 2 (obtained by multiplying the weights of base model 2 by the found couplings) and base model 1 lie close to each other and are separated by a low energy barrier. These visualizations thus provide new empirical evidence in support of the conjecture made in \cite{entezari2021role}. They also shed light on the workings on WB fusion algorithm. In particular, equation \ref{eq: update formula for W_l} can be interpreted as coordinate-wise averaging of the permuted models. Since permuted models land in basins that are separated by low energy barriers, their linear interpolation gives a good fused model.


\begin{figure}[!htb]
    \centering
    \begin{subfigure}{.33\textwidth}%
    \includegraphics[width=1.0\linewidth]{pics/test_error_plane_VGG11_CIFAR10.pdf}
    \end{subfigure}%
    \begin{subfigure}{.33\textwidth}%
    \includegraphics[width=1.0\linewidth]{pics/test_error_plane_LSTM_MNIST.pdf}
    \end{subfigure}%
    \begin{subfigure}{.33\textwidth}%
    \includegraphics[width=1.0\linewidth]{pics/test_error_plane_LSTM_DBpedia.pdf}
    \end{subfigure}
\caption{Visualizations of the fusion results on the test error surface, which is a function of network weights in a two-dimensional subspace, for different models and datasets. \textbf{Left:} Fusion of two VGG11 models trained on CIFAR10 dataset using WB framework. \textbf{Middle:} Fusion of two LSTM models trained on MNIST dataset . \textbf{Right:} Fusion of two LSTM models trained on DBpedia dataset. We can observe that in all these cases the basins of permuted model $2$ (obtained by multiplying the weights of base model $2$ by the found coupling) and base model 1
lie close to each other and are separated by a low energy barrier.}
% \textit{after} multiplying the couplings found by our fusion algorithm, base model 2 will end up lying in the basin that close to one model 1 lands in.}
\label{fig: visualization of fusion results for different types of models and datasets}
\end{figure}

\subsection{GWB fusion for recurrent neural networks}\label{sec: experiments on GWB based fusion}
{\textbf{Setup:}
In this section, we consider the fusion of NNs like RNNs and LSTMs on sequence based tasks. 
We use 4 different datasets for this setting: 
i) MNIST \cite{deng2012mnist}: Images of $28\times 28$ dimensions are interpreted as $28$ length sequences of vectors $\in \mathbb{R}^{28}$; 
ii) SST-2 \cite{socher2013recursive}: Binary classification task of predicting positive and negative phrases; 
iii) AGNEWS \cite{zhang2015character}: Corpus of news articles from 4 classes;
and iv) DBpedia \cite{zhang2015character}: Ontology classification dataset containing 14 non-overlapping classes. 
% The base models are RNNs and LSTMs with one hidden layer and 
% hidden dimensions of size $256$ and $4\times 256$ respectively. 
For the NLP tasks, we use pre-trained GloVe embeddings \cite{pennington2014glove} of dimensions $100$ and $50$
for RNNs and LSTMs respectively. 
The embedding layer is not updated during the model training.
We set the target model to have the same architecture as the base models.
}
%{\red \textbf{Setup:} In this section, we show the importance of utilizing the hidden-to-hidden weights of RNN during the fusion by comparing the performance of GWB based fusion algorithm with other fusion types. We consider $4$ different tasks for the experiments on RNN and LSTM models. Specifically, the $4$ datasets are: i) MNIST dataset; ii) AGNEWS dataset ..; iii) DBpedia dataset ..; iv) SST dataset .. . In general, the base models are RNNs and LSTMs with one hidden layer. The hidden dimensions of RNN and LSTM models are $256$ and $4 \times 256$ respectively. For the image task (MNIST dataset), the input dimension and the time step of RNN and LSTM are set to be $28$, which fits the size of the digital image in MNIST; for the NLP tasks (AGNEWS, DBpedia, SST datasets), we consider RNN and LSTM models consisting of a pre-trained embedding layer (embedding vary for different datasets, see the detailed settings of both image and NLP tasks in the Supplement). We set target model to have the same architecture as the base models. And when conducting fusion on NLP datasets, we assume that the target model shares the same pre-trained embedding with base models.}

{\textbf{Quantitative results:} Table \ref{table: GWB fusion comparison} contains the result of fusion for various datasets and model architectures. We find that 
(a) our GWB framework outperforms other fusion algorithms for each combination of model type and dataset, 
which highlights the importance of using hidden-to-hidden connections for the fusion of recurrent NNs; 
(b) the accuracy gains for GWB over WB is different for different tasks, 
which indicates that relative importance of hidden-to-hidden connections is task dependent; 
(c) the accuracy of fused model is higher for LSTMs in comparison to RNNs,
which we attribute to the fact that LSTMs have four hidden states 
and thus four input-to-hidden and hidden-to-hidden weight matrices. 
More information for each hidden node allows the algorithm to uncover better couplings.
Our results in (a) and (b) show the usefulness of hyperparameter $\alpha_H$ (set between $[1,20]$) from \eqref{eq: GWBP for rnn fusion}
in balancing the relative importance of hidden-to-hidden weights. 
% In our experiments,
% we find that setting $\alpha_H \in [1, 20]$ 
% results in better fused model for GWB. 
}
%{\red \textbf{Quantitative Results:} Table \ref{table: GWB fusion comparison} contains result of comparisons between GWB basd fusion with other fusion types on different network architectures and datasets. (a) Our GWB framework outperforms other fusion algorithms for each combination of model type and dataset, which demonstrates the importance of using hidden-to-hidden weights during the RNN fusion. (b) We observe that, for the MNIST and DBpedia datasets, using GWB framework will boost the accuracy compared to WB based fusion; while for the AGNEWS and SST datasets, the difference are not substantial. This might indicate that the importance of hidden-to-hidden weights varies for different tasks. Moreover, when considering fusion on MNIST and DBpedia datasets using GWB framework, we find out that setting hyperparameter $\alpha_H$ in \eqref{eq: GWBP for rnn fusion}, which balances the importance of input-to-hidden and hidden-to-hidden weights, to be relatively large (like $100$ or $1000$) will usually give us better fusion results compared to choosing small value of $\alpha_H$ (WB fusion can be thought as the case $\alpha_H=0$; see more detailed hyperparameter choosing in the Supplement). However, different choices on $\alpha_H$ will not have large affect on results of GWB fusion on datasets AGNEWS and SST. (TODO: Explanations or insight).  (c) We observe that, for each dataset, while the difference between base models' accuracy for RNNs and LSTMs are small, the fused models of LSTM perform much better than RNN. Since the hidden dimension of base LSTM models are $4$ times larger than base RNN models, we think the difference on the fused models might related to the mean-field limit of neural networks \cite{mei2018mean}. This connection for the fully connected NNs has been explored in \cite{singh2019model}, we leave more explorations on RNN cases using our framework in the future work.}
 
\begin{table}[htb]
	\caption{Performance comparison (Test accuracy $\pm$ standard deviation \%) of different fusion algorithms under various network architectures and datasets. For each case, target model obtained by GWB fusion reaches the highest test accuracy and small standard deviation.}
	\label{table: GWB fusion comparison}
	\centering
	\renewcommand\arraystretch{1.5}
	%	\setlength{\abovecaptionskip}{0pt}%    
	%	\setlength{\belowcaptionskip}{10pt}%
	%\resizebox{0.5\textwidth}{0.09\textwidth}{
	\resizebox{1.0\textwidth}{!}{
		\begin{sc}
			\begin{tabular}{@{}cccccccccccc@{}}
				%\toprule
				& \multicolumn{2}{c}{MNIST} & \phantom{ab}& 
				\multicolumn{2}{c}{AGNEWS} &
				\phantom{ab}&
				\multicolumn{2}{c}{DBpedia} &
				\phantom{ab}&
				\multicolumn{2}{c}{SST-2}\\ 
				\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}
				&  RNN & LSTM&  & RNN & LSTM & & RNN & LSTM & & RNN & LSTM \\ 
				\midrule
				Base Model Avg & $96.68 \pm 0.29$ & $98.99 \pm 0.09$ &  & $88.68 \pm 0.12$& $92.38 \pm 0.17$& & $97.12 \pm 0.21$ & $98.62 \pm 0.11$ & & $87.32 \pm 1.03$& $90.31 \pm 0.27$\\
				\midrule[0.05pt]
				Vanilla Avg & $28.54 \pm 10.70$ & $31.92 \pm 4.86$ &  & $40.77 \pm 4.94$& $74.01 \pm 3.89$& & $30.95 \pm 4.53$& $50.93 \pm 2.17$ & & $73.91 \pm 2.73$& $74.25 \pm 1.92$\\
				OT & $36.78 \pm 14.13$ & $68.33 \pm 7.07$ &  & $53.05 \pm 4.30$& $86.19 \pm 2.14$& & $37.91 \pm 4.86$& $77.95 \pm 3.20$ & & $78.92 \pm 2.97$& $82.13 \pm 0.60$\\
				One-shot FedMA & $34.16 \pm 7.26$ & $66.98 \pm 5.17$ & & 
				$55.78 \pm 3.64$ & $86.30 \pm 2.40$ & &
				$42.16 \pm 6.24$ & $81.81 \pm 3.29$ & &
				$79.17 \pm 2.27$ & $82.53 \pm 1.01$ \\
				WB  & $29.41 \pm 7.05$ & $67.66 \pm 6.27$ &  & $55.63 \pm 4.18$ &  $86.25 \pm 2.37$ &  & $42.52 \pm 6.26$& $82.57 \pm 3.55$ & & $79.57 \pm 2.36$ & $82.87 \pm 1.09$\\
				GWB & $\bm{81.39 \pm 2.97}$ & $\bm{93.27 \pm 1.86}$ & & $\bm{61.01 \pm 3.87}$ & $\bm{87.96 \pm 0.91}$ & & $\bm{55.15 \pm 5.97}$& $\bm{87.50 \pm 2.89}$ & & $\bm{82.60 \pm 1.05}$ & $\bm{84.04 \pm 0.77}$\\
				\bottomrule
			\end{tabular}
		\end{sc}
	}
\end{table}

\textbf{Visualizations:} Figure \ref{fig: visualization of fusion results for different types of models and datasets} (middle, right) 
contains visualization of fusing LSTM models under the GWB framework. 
{As noted for the FC NNs and deep CNNs visualizations, we find that (a) the couplings found by GWB fusion algorithm 
are sparse, and (b) these couplings map different local minima into neighboring basins 
that are separated by low energy barriers. }
This empirical evidence suggests that the original conjecture in \cite{entezari2021role}
can be extended to richer network architectures and tasks (RNNs and LSTMs on NLP datasets).  









==> Wasserstein Barycenter-based Model Fusion and Linear Mode Connectivity of Neural Networks/macros.tex <==
\newcommand{\mlp}{\textsc{MLPNet}}
\newcommand{\mlps}{\textsc{MLPSmall}}
\newcommand{\mlpl}{\textsc{MLPLarge}}
\newcommand{\resnet}{\textsc{ResNet18}}
\newcommand{\vgg}{\textsc{VGG11}}

==> Wasserstein Barycenter-based Model Fusion and Linear Mode Connectivity of Neural Networks/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Wasserstein Barycenter-based Model Fusion and Linear Mode Connectivity of Neural Networks/resnet.tex <==
\subsection{Extension to ResNets}\label{subsec: extension to ResNets}
%For common fully connected or convolutional neural networks, layer $N_l^i$ is supported on the previous layer $N_{l-1}^i$. 

%\begin{wrapfigure}{R}{0.5\textwidth}
%	\vspace{-12pt}
%	\centering
%	\includegraphics[width=0.5\textwidth]{pics/resnet.png}
%	\caption{A building block of ResNet. Due to skip connection, 
%		outputs $X_1^i$ and $X_3^i$ of layers $N^i_1$ and $N^i_3$ gets added up
%		before feeding into layer $N^i_4$.}
%	\label{fig: ResNet's building block}
%	\vspace{-25pt}
%\end{wrapfigure}

{ResNet models are neural networks that contain skip connections
	 that ``jump'' over some layers to avoid the problem of vanishing gradients. Figure \ref{fig: ResNet's building block} shows a typical building block 
 	of a ResNet model. 
 	For a layer $N_l$ we let $\mathcal{C}_l=\{N_{\alpha}\}_{\alpha \in \Lambda}$ be the collection of all the previous layers that connect with it. Since the outputs of layers in $\mathcal{C}_l$ are added up before 
 	feeding them into layer $N_l$,  skip connections constrain the layers 
 	in $\mathcal{C}_l$ to share the same coupling, i.e $\Pi_\alpha=\Pi^*\; \forall \alpha$. This constraint allows us to use any of the previous layers in $\mathcal{C}_l$
	as the support for $N_l$ since they share the same coupling $\Pi^*$ 
	and hence produce the same cost to be used in optimization \eqref{eq: problem after plugging in cost function d_W}. Our convention is to find a coupling for the earliest layer 
	in $\mathcal{C}_l$ first and then use the same coupling when we fuse the other layers in $\mathcal{C}_l$ .
} 




%\begin{figure}[htbp]
%	%\vspace{-12pt}
%	\centering
%	\includegraphics[width=0.6\textwidth]{pics/resnet.png}
%	\caption{A building block of ResNet. Due to skip connection, 
%		outputs $X_1^i$ and $X_3^i$ of layers $N^i_1$ and $N^i_3$ gets added up
%		before feeding into layer $N^i_4$.}
%	\label{fig: ResNet's building block}
%	%\vspace{-25pt}
%\end{figure}


%\begin{figure}[htbp]
%	\centering
%	\begin{subfigure}[b]{0.49\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{pics/cnn1.jpeg}
%		\caption{CNN.}
%		\label{fig: CNN example}
%	\end{subfigure}
%    \hfill
%    \begin{subfigure}[b]{0.49\textwidth}
%    	\centering
%    	\includegraphics[width=\textwidth]{pics/resnet1.jpeg}
%    	\caption{ResNet.}
%    	\label{fig: ResNet's building block}
%    \end{subfigure}
%    \caption{\textbf{Left:} A channel $v^i_{l,1}$ in the convolutional layer $N_l^i$ is interpreted as a node in our framework, with weight function $W^i_{l,1}$ mapping previous layer elements (channels) to $\R^{k\times k}$. \textbf{Right:} A building block of ResNet. Due to skip connection, outputs $X_1^i$ and $X_3^i$ of layers $N^i_1$ and $N^i_3$ gets added up before feeding into layer $N^i_4$.}
%\end{figure}















